Dark Energy with a Triplet of Classical U(1) Fields

We present a new mechanism for cosmic acceleration consisting of a scalar field coupled to a triplet of classical U(1) gauge fields. The gauge fields are arranged in a homogeneous, isotropic configuration, with both electric- and magnetic-like vacuum expectation values. The gauge fields provide a mass-like term via a Chern-Simons interaction that suspends the scalar away from its potential minimum, thereby enabling potential-dominated evolution. We show this mechanism can drive a brief period of acceleration, such as dark energy, without the need for fine tunings. We obtain simple analytic results for the dark energy equation of state and dependence on model parameters. In this model, the presence of the gauge field generically leads to a suppression of long-wavelength gravitational waves, with implications for the experimental search for cosmic microwave background B-modes and direct detection of a stochastic gravitational wave background.

==> scenario.tex <==
We describe two potential scenarios for the origin of the electric and magnetic vevs.

The first scenario is a form of gauge field inflation with a flavor-space locked field $A^a_i = \phi(t) \delta^a_i$. Over the course of inflation, the gauge field is amplified until $F^{a}_{\mu\nu}$ has non-zero electric (0i) and magnetic (jk) components. 

After inflation, one could follow the evolution of the SU(2) fields and look for the impact on primordial gravitational waves. However, there are two difficulties in this case. First, the Yang-Mills coupling needed for successful inflation will cause the gauge fields to oscillate soon after the end of inflation, thereby erasing the electric and magnetic vevs. Another problem is that the coupling will run and lead to confinement. These are both interesting features of the scenario, but if we are interested in the survival of the vevs, they should transfer to a U(1). 

Hence, we consider the spontaneous symmetry breaking from SU(2) to U(1) near the end of inflation. Two of the bosons acquire mass, but the third remains massless. The vevs associated with the two massive bosons vanish; those components of the massive gauge field will rapidly oscillate. This leaves the vevs of the massless boson consisting of uniform, colinear electric and magnetic fields. 

In terms of stress-energy tensor, the single pair of colinear fields is not isotropic. Hence, we need two more SU(2) or some suitably large SU(N) to break to three U(1)s. Each will produce a pair of colinear fields, which will not be mutually orthogonal. However, evolving in a homogeneous, isotropic spacetime, the anisotropic portion of the field configurations will decay more rapidly than the isotropic portion. In a short amount of time, the surviving fields will be the isotropic, homogeneous configuration of three flavors of colinear electric and magnetic vevs.

# Open questions: are the massive gauge bosons charged under the photon? does the existence of a magnetic monopole solution affect the scenario?

# In the SM SU(2)xU(1)->U(1) case, the W bosons are charged, but there are no monopoles. Can the SU(2)->U(1) case circumvent the charge bosons, or can the SU(2)xU(1)->U(1) case avoid charged W-like bosons by some other means?


The second scenario is based on inflationary magnetogenesis scenarios in which conformal invariance of a U(1) is broken and exploited to amplify a primordial magnetic field. For simplicity, we consider a massive U(1) which will later undergo symmetry restoration. In the broken phase, fluctuations are amplified and exit the horizon. The collection of modes that exit the horizon before the final 60 e-foldings of inflation will be effectively homogeneous. 

# The problem is that there is nothing to select a particular direction, and so the effect will average out to zero.

# Why are galaxy-scale B fields not also washed out in these magnetogenesis scenarios?
 
